A new meteor shower from comet 46P/Wirtanen expected in December 2023

Context. Comet 46P/Wirtanen is a near-Earth object (NEO) for which no associated meteor shower has ever been reported. Aims. This study is aimed at improving our understanding of why there has been no observed shower activity for this NEO to date, as well as to consider whether any past activity could be uncovered from the post-prediction results. Methods. The usual dynamic tools for meteoroid streams were used to describe the behavior of the particles ejected by the comet. The resulting modeled meteoroid stream was thoroughly inspected for collisions between the stream and the Earth. Results. The results show a possible encounter forecast for December 12, 2023, between 8:00 and 12:30 UT. The slow entry velocity is typically known to cause dim meteors. The activity level of the shower is highly uncertain due to the absence of reported past showers. Conclusions. Overall, the most optimal observations on the forecasted day would be achieved from Eastern Australia, New Zealand, and Oceania. These observations will help constrain the size distribution of meteoroids from comet 46P/Wirtanen in the millimeter range.

==> Danielle/method_reorg.tex <==
The methods used are based on similar previous studies of the dynamics of meteoroid streams and its application to the forecast of meteor showers \citep{YeVaubaillon2021,YeVaubaillon2022}. In this case, several different models are considered. For each model, simulated meteoroids were ejected from 46P/Wirtanen at each return of the comet and integrated until the present epoch to analyze the current dust distribution near the Earth. Details about the simulation parameters used are presented in Table~\ref{tab:model_parameters}.

One model used was developed by \cite{Ye2016}; this model tested classical pure-ice model \citep{Whipple1950} with ejection speeds multiplied by $0.1\times$, $1\times$ and $5\times$ in order to cover different activity levels of the parent comet. 

Another model is based on \cite{Vaubaillon2005a,Vaubaillon2005b}. The comet perihelion passages taken into account here are restricted to the observed ones, i.e. since 1954. \addae{The dust production rate was calculated using the measured $Af\rho=150$~cm, where $Af\rho$ is a proxy of dust production \citep{AHearn1984}.}

Additional simulations were conducted based on the model of \cite{Egal2019}. Several simulations were performed to investigate the influence of the diameter of the nucleus and the fraction of active area (from 20\% to 40\%). \addae{In conjunction with these independent simulations we tested two different dust size distributions for the comet, } characterized by the differential size indices $\alpha_\mathrm{d}=3.3$ as found by \citet{Protopapa2021} which is in line with typical comets \citep{Fulle2004}, and the unusually steep $\alpha_\mathrm{d}=5.9$ found by \citet{Kareta2023}. 
%(here $\alpha_\mathrm{d}$ is the differential dust size index.) 

\adddm{The model of \cite{Moser2004EMP,Moser2008EMP} was used in a fourth simulation, taking into account perihelion passages since 1900 and utilizing the meteoroid ejection model of \citep{Jones1996ASPC137}.  The active area fraction was set at 50\%.}
